Digital Twin Catalog: A Large-Scale Photorealistic 3D Object Digital Twin Dataset

We introduce the Digital Twin Catalog (DTC), a new large-scale photorealistic 3D object digital twin dataset. A digital twin of a 3D object is a highly detailed, virtually indistinguishable representation of a physical object, accurately capturing its shape, appearance, physical properties, and other attributes. Recent advances in neural-based 3D reconstruction and inverse rendering have significantly improved the quality of 3D object reconstruction. Despite these advancements, there remains a lack of a large-scale, digital twin-quality real-world dataset and benchmark that can quantitatively assess and compare the performance of different reconstruction methods, as well as improve reconstruction quality through training or fine-tuning. Moreover, to democratize 3D digital twin creation, it is essential to integrate creation techniques with next-generation egocentric computing platforms, such as AR glasses. Currently, there is no dataset available to evaluate 3D object reconstruction using egocentric captured images. To address these gaps, the DTC dataset features 2,000 scanned digital twin-quality 3D objects, along with image sequences captured under different lighting conditions using DSLR cameras and egocentric AR glasses. This dataset establishes the first comprehensive real-world evaluation benchmark for 3D digital twin creation tasks, offering a robust foundation for comparing and improving existing reconstruction methods. The DTC dataset is already released at https://www.projectaria.com/datasets/dtc/ and we will also make the baseline evaluations open-source.

==> tbl_text/baseline_aria_geometry.tex <==
\begin{table}[t]
\centering
\small
\caption{Benchmarking appearance and geometry reconstruction of egocentric aligned digital twin recordings.}
\begin{tabular}{cccc}
\toprule
      & PSNR $\uparrow$ & Depth $\downarrow$  & Normal $\downarrow$  \\ \midrule
3D-GS \citep{kerbl3Dgaussians} & 29.83 & 0.1505 & 0.3334 \\
2D-GS \cite{huang20242Dgs} & 29.54 & 0.1474 & 0.1509 \\
\bottomrule
\end{tabular}

\label{tab:aria_geometry}
\end{table}

==> text/6_supp_old.tex <==
1. Dataset statistics (3D object category list, object list used in DSLR recording \& aria recordings), more visual examples for 3D objects (PBR), real world recording examples and aria recordings.

2. Benchmark:
    Sparse-view --> LRM (both DSLR and Ego)
    Dense-view --> Neural-PBIR
    Robotic experiment details?   
    Need to spend some time looking at the results for each baseline method, and write a simple result analysis for each baseline. Try to pick up the challenging results that existing work that do not work well and can be surfaced by our evaluation. 
    Need to add shape ground truth evaluation using metrics consistent with the DSLR evaluation. 

3. Dataset processing pipeline description 
    More details on the decisions and results for the dataset generation (alignment) process. 

4. Put a video to highlight digital twin assets. 
    * Fix the color tone mismatch in the current comparison videos. 
    * To show the raw video footage.
